PH-Net: Parallelepiped Microstructure Homogenization via 3D Convolutional Neural Networks

Microstructures are attracting academic and industrial interests with the rapid development of additive manufacturing. The numerical homogenization method has been well studied for analyzing mechanical behaviors of microstructures; however, it is too time-consuming to be applied to online computing or applications requiring high-frequency calling, e.g., topology optimization. Data-driven homogenization methods emerge as a more efficient choice but limit the microstructures into a cubic shape, which are infeasible to the periodic microstructures with a more general shape, e.g., parallelepiped. This paper introduces a fine-designed 3D convolutional neural network (CNN) for fast homogenization of parallel-shaped microstructures, named PH-Net. Superior to existing data-driven methods, PH-Net predicts the local displacements of microstructures under specified macroscope strains instead of direct homogeneous material, motivating us to present a label-free loss function based on minimal potential energy. For dataset construction, we introduce a shape-material transformation and voxel-material tensor to encode microstructure type,base material and boundary shape together as the input of PH-Net, such that it is CNN-friendly and enhances PH-Net on generalization in terms of microstructure type, base material, and boundary shape. PH-Net predicts homogenized properties with hundreds of acceleration compared to the numerical homogenization method and even supports online computing. Moreover, it does not require a labeled dataset and thus is much faster than current deep learning methods in training processing. Benefiting from predicting local displacement, PH-Net provides both homogeneous material properties and microscopic mechanical properties, e.g., strain and stress distribution, yield strength, etc. We design a group of physical experiments and verify the prediction accuracy of PH-Net.

==> data.tex <==
\section{Dataset Generation}
\label{sec:dataset}



\subsection{Selection of parameters}
We consider three distinct types of parameters in dataset construction: shape, microstructure, and base material.



\subsubsection{Shape parameters}
 To reduce the complexity of deformed microstructure homogenization, we assume all microstructures that belong to our dataset are limited to parallel hexahedra.
Then, we search the optimal pairs from deformed hexahedra to parallel hexahedra by geometry processing, e.g., iterative closest point algorithm~\cite{paulj1992method}, to minimize matching errors. 

Thanks to parallelism, any deformed hexahedron $Q$ in the dataset can be derived from a cubic unit $P$, whose orthogonal coordinate system is deformed into a non-orthogonal basis by a linear transformation.
As shown in Figure~\ref{fig:parameters}, the linear mapping $F:P \to Q$ is parameterized by 6 variables, which are the magnitude scales of coordinate axes and the angles between them.
We use $l_x, l_y, l_z$ and $\alpha_{xy}, \alpha_{yz}, \alpha_{xz}$ to denote the scale variables and angle variables, respectively. 

In this paper, we set scale variables $l_x,l_y,l_z\in[\frac{2}{3},\frac{3}{2}]$ and angle variables $\alpha_{xy}, \alpha_{yz}, \alpha_{xz} \in[75^{\circ},90^{\circ}]$
To eliminate rotational errors, we specify that the X-axis of the deformed hexahedron is $[1,0,0]^T$, and the $X-Y$ plane is perpendicular to $[0,0,1]^T$.
Therefore, we can express the mapping relationship as the product of the scaling matrix $T(l_x,l_y,l_z)$ and the shear matrix $S(\alpha_{xy}, \alpha_{yz}, \alpha_{xz})$, that is $F = ST$. 
Similarly, we can calculate linear mapping $G:Q\to P$ by inversing $F$ in turn.

\begin{figure}
    \centering
    \includegraphics[width=.7\linewidth]{figure/parameters.jpg}
    \centerline{\scriptsize Cubic unit $P$ \hspace{0.2\linewidth}Parallel hexahedron $Q$ }
    \caption{The linear map $F$ and its inverse $G$ between cubic unit $P$ and parallel hexahedron $Q$ are considered as the transformation of coordinate basis with three scaling variables $l_x,l_y,l_z$ and three angle variables $\alpha_{xy},\alpha_{yz},\alpha_{zx}$, respectively.}
    \label{fig:parameters}
\end{figure}

\subsubsection{Microstructure parameter and its base material}
For a given microstructure $\Omega$ in the dataset, regardless of its geometric parameters, it is voxelized into a 0-1 3D tensor, whose size is $N^3$. It is divided into two parts, of which the solid part is 1. To be specific, the usage of our approach is limited to linear elasticity. Therefore, we implement isotropic material $C^b(E,v)$ as the base material in the dataset, which can be easily calculated by Young's modulus $E$ and Poisson ratio $v$.

However, using only the solid part as input in the 3D CNN training will result in incorrect output. That is because some weights in the neural network lack backward gradients so that they are never updated. Hence, we have to assume that the microstructure in the dataset is composed of a two-phase composite of hard and soft materials, in which the hard material property $C^{bh}$ is set to $E=1, v=0.3$, but the soft one $C^{bs}$ is set to $E=10^{-6}, v=0.3$. 


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{figure/transformation.jpg}
    \caption{(a) In dataset construction, a deformed microstructure with an isotropic base material $C^b$ is converted into a normal microstructure with a  transformed base material $\tilde C^b$ by shape-material transformation; (b) the inverse procedure after computing the homogenized material properties $\tilde C^H$ of the cubic unit, aims to recover the homogenized material $C^H$ on the parallel hexahedron.
    } 
    \label{fig:shape_to_material}
\end{figure*}

\subsection{Shape-material transformation}
\label{sec:transformation}
As we know, there has not been a deep learning method used to predict the macroscope properties of deformed microstructures up to now. Most DL methods for predicting microstructure properties require voxel-based inputs for their innately fit for DL operations, like \textit{conv} and \textit{pooling}. However, deformed microstructures lose this edge. 



As mentioned above, shape deformation $F:P\to Q$ can be considered as a non-orthogonal basis, in which a hexahedron $Q$ is expressed as a cubic unit. 
If displacements $u$ satisfy the elastic equation $K(C)u=f$ on a unit domain, $\tilde{u}$ and $\tilde{f}$ are the displacement and force expressed on the non-orthogonal basis, respectively, Tozonoi~\etal have proved that they also satisfy the elastic equation
\begin{equation}
    \tilde K(\tilde C)\tilde u=\tilde f,
    \label{equ:deformed_elastic_quation}
\end{equation}

only if the base material $C^b$ is transformed by
\begin{equation}
    \tilde{C}^b_{ijkl}=G_{pi}G_{qj}G_{rk}G_{sl}C^b_{pqrs}, 
    \label{equ:pqrs1}
\end{equation}
where $G:Q \to P$ is the inverse map from a hexahedron to a cubic unit. This can be verified directly by changing variables in Eq.~\ref{equ:Ku=f}. Also, the homogenized elastic tensor $C^H$ can be expressed in terms of $\tilde{C}^H$ by the inverse relation:
\begin{equation}
    C^H_{ijkl}=F_{pi}F_{qj}F_{rk}F_{sl}\tilde{C}^H_{pqrs}.
    \label{equ:pqrs2}
\end{equation}

Therefore, the whole processing of DH-Net works as follows:
\begin{enumerate}
    \item Compute $\tilde{C}^{bh}$ and $\tilde{C}^{bs}$ by Eq.~\ref{equ:pqrs1}, then construct $\tilde C^{bh}\times\Omega+\tilde C^{bs}\times(1-\Omega)$ as input (Figure~\ref{fig:shape_to_material}a);
    \item Predict microscope displacements $\tilde u$ using DH-Net, and calculate homogenized elastic tensor $\tilde C^H$;
    \item Recover homogenized tensor $C^H$ on the orthogonal basis by Eq.~\ref{equ:pqrs2} (Figure~\ref{fig:shape_to_material}b).
\end{enumerate}



\subsection{Dataset Construction}
For each input to DH-Net, we first transform base materials $\tilde C^{bh}$ and $\tilde C^{bs}$ and reshape each base material ($6\times6$ elastic tensor) into a vector, then combine the microstructure $\Omega$ with its base materials by $C^{bh}\times\Omega+C^{bs}\times(1-\Omega)$, whose size is $N^3\times 36$. 
We construct the dataset by sampling each shape parameter 5 times at equal intervals.

We adopt a typical microstructure, Tubular Gyroid (TG), a type of triply periodic minimal surface (TPMS) in the dataset and  uniformly sample the TG structure 40 times with the volume fraction within $[2.4\%,33\%]$.
Combined with the shape parameters, the dataset is of $625$K samples, which leads extraordinarily time-consuming training process.
So we performed experiments on randomly pruning the dataset into $1\%$, $5\%$ and $10\%$ sets, and found that the dataset with $10\%$ random sample points (totally 62.5K) achieved the excellent balance of convergences and prediction errors.


